Gaussian Process-Augmented Model Predictive Contouring Control for 6-DoF Trajectory Tracking with a Holonomic AUV

Small, holonomic Autonomous Underwater Vehicles (AUVs) enable close-range inspection of underwater structures from arbitrary viewpoints, requiring accurate position and attitude tracking under state and input constraints. Model Predictive Contouring Control (MPCC) naturally handles these requirements, but relies on an accurate dynamics model, which is difficult to obtain underwater. In this paper, we present a nonlinear MPCC in all six Degrees of Freedom (DoF) for a holonomic AUV and alleviate the inaccuracies in the dynamics by augmenting the nominal model employed with residual dynamics learned via Gaussian Process (GP) regression. The learned residual is embedded in the optimal control problem through a zero-order robust optimization scheme, which keeps the controller real-time capable at 25 Hz. A simulation ablation shows that residual selection is essential when designing the controller, and simulation and in-water experiments with the Multimodality, Observing, Low-cost, Agile (MOLA) AUV validate the resulting controllers against a nominal MPCC and a field proven Proportional-Integral-Derivative (PID) controller.

==> tex-utils/glossary.tex <==
%------------------------------------------------------------------------------%
% List of all acronyms used somewhere
%------------------------------------------------------------------------------%

%-----A-----%
\newacronym{adcp}{ADCP}{Acoustic Doppler Current Profiler}
\newacronym{agv}{AGV}{Autonomous Ground Vehicle}
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{aoa}{AoA}{Angle of Attack}
\newacronym{aop}{AOP}{Apparent Optical Property}
\newacronym{auv}{AUV}{Autonomous Underwater Vehicle}
\newacronym{ar}{AR}{Augmented Reality}
\newacronym{ard}{ARD}{Automatic Relevance Determination}
\newacronym{asv}{ASV}{Autonomous Surface Vehicle}

%-----B-----%
\newacronym{bdi}{BDI}{Beliefs Desires Intentions}
\newacronym{bo}{BO}{Bayesian Optimization}
\newacronym{bt}{BT}{Behavioural Tree}
%-----C-----%
\newacronym{cad}{CAD}{Computer Aided Design}
\newacronym{can}{CAN}{Controller Area Network}
\newacronym{cb}{CB}{Center of Buoyancy}
\newacronym{cbf}{CBF}{Control Barrier Function}
\newacronym{cf}{CF}{Center of flotation}
\newacronym{cfd}{CFD}{Computational Fluid Dynamics}
\newacronym{cg}{CG}{Center of Gravity}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{co}{CO}{Coordinate origin}
\newacronym{cog}{CoG}{Center of Gravity}
\newacronym{cps}{CPS}{Cyber-Physical System}
\newacronym{cpu}{CPU}{Central Processing Unit}
\newacronym{cr}{CR}{Center of Rotation}
\newacronym{ctd}{CTD}{Conudctivity, Temperature, Depth}

%-----D-----%
\newacronym{dig}{DIG}{Dynamic Interaction Graph}
\newacronym{dnf}{DNF}{Decentralized Navigation Function}
\newacronym[longplural={Degrees of Freedom},shortplural={DoF}]{dof}{DoF}{Degree of Freedom}
\newacronym{dqn}{DQN}{Deep Q-Learning Network}
\newacronym{dr}{DR}{Dead Reckoning}
\newacronym{drl}{DRL}{Deep Reinforcement Learning}
\newacronym{dvl}{DVL}{Doppler Velocity Log}

%-----E-----%
\newacronym{ecef}{ECEF}{Earth-centered Earth-fixed (frame)}
\newacronym{eci}{ECI}{Earth-centered inertial (frame)}
\newacronym{ekf}{EKF}{Extended Kalman Filter}
\newacronym{enu}{ENU}{East-North-Up}
\newacronym{erm}{ERM}{Empirical Risk Minimization}

%-----F-----%
\newacronym{frd}{FRD}{Forward-Right-Down}
%-----G-----%
\newacronym{gis}{GIS}{Geographical Information System}
\newacronym[longplural={Gaussian Processes}]{gp}{GP}{Gaussian Process}
\newacronym{gpr}{GPR}{Gaussian Process Regression}
\newacronym{gps}{GPS}{Global Positioning System}
\newacronym{gpu}{GPU}{Graphical Processing Unit}
\newacronym{grv}{GRV}{Gaussian Random Variable}

%-----H-----%
\newacronym{hil}{HIL}{Hardware-in-the-Loop}
%-----I-----%
\newacronym{ibvs}{IBVS}{Image-Based Visual Servoing}
\newacronym{imu}{IMU}{Inertial Measurement Unit}
\newacronym{ins}{INS}{Inertial Navigation System}
\newacronym{iop}{IOP}{Inherent Optical Property}
\newacronym{iss}{ISS}{Input-to-State Stability}
\newacronym{isss}{ISSS}{Interferometric Side Scan Sonar}
%-----J-----%
%-----K-----%
%-----L-----%
\newacronym{lars}{LARS}{Launch and Recovery System}
\newacronym{lbl}{LBL}{Long Baseline}
\newacronym{lcf}{LCF}{Longitudinal Center of Flotation}
\newacronym{lcg}{LCG}{Longitudinal Center of Gravity}
\newacronym{lcm}{LCM}{Lightweight Communications and Marshalling}
\newacronym{lm}{LM}{Levenberg-Marquardt}
\newacronym{lqg}{LQG}{Linear Quadratic Gaussian}
\newacronym{lqr}{LQR}{Linear Quadratic Regulator}
\newacronym{lti}{LTI}{Linear Time Invariant}
\newacronym{ltv}{LTV}{Linear Time Varying}
\newacronym{lut}{LUT}{Look-Up Table}
\newacronym{lvs}{LVS}{Laser Vision System}

%-----M-----%
\newacronym{mbari}{MBARI}{Monterey Bay Aquarium Research Institute}
\newacronym{mbes}{MBES}{Multi-Beam Echo Sounder}
\newacronym{mcts}{MCTS}{Monte Carlo Tree Search}
\newacronym{mdp}{MDP}{Markov Decision Process}
\newacronym{mimo}{MIMO}{Multi-input Multi-output}
\newacronym{ml}{ML}{Machine Learning}
% \newacronym{mola}{6-DoF}{}
% \glsunset{mola}
\newacronym{mola}{MOLA}{Multimodality, Observing, Low-cost, Agile}
\newacronym{mpc}{MPC}{Model Predictive Control}
\newacronym{mpcc}{MPCC}{Model Predictive Contouring Control}
\newacronym{mse}{MSE}{Mean Squared Error}

%-----N-----%
\newacronym{naf}{NAF}{Normalized Advantage Functions}
\newacronym{ned}{NED}{North-East-Down}
\newacronym{nfq}{NFQ}{Neural Fitted Q Iteration}
\newacronym{nmpc}{N-MPC}{Non-linear Model Predictive Control}
\newacronym{nn}{NN}{Neural Network}
\newacronym{nse}{NSE}{Navier-Stokes Equation}

%-----O-----%
\newacronym{ocp}{OCP}{Optimal Control Problem}
\newacronym{ode}{ODE}{Ordinary Differential Equation}
%-----P-----%
\newacronym{pac}{PAC}{Probably Approximately Correct}
\newacronym{pbvs}{PBVS}{Position-Based Visual Servoing}
\newacronym{pd}{PD}{Proportional-Derivative}
\newacronym{pi}{PI}{Proportional-Integral}
\newacronym{pid}{PID}{Proportional-Integral-Derivative}
\newacronym{pilco}{PILCO}{Probabilistic Inference for Learning Control}
\newacronym{piml}{PIML}{Physics-informed Machine Learning}
\newacronym{pnp}{PnP}{Perspective-n-Point}
\newacronym{proxop}{ProxOp}{Proximity Operation}
\newacronym{pwm}{PWM}{Pulse-Width Modulation}
%-----Q-----%
%-----R-----%
\newacronym{ram}{RAM}{Random Access Memory}
\newacronym{ransac}{RANSAC}{Random Sample Consensus}
\newacronym{rl}{RL}{Reinforcement Learning}
\newacronym{rms}{RMS}{Root Mean Square}
\newacronym{rmse}{RMSE}{Root Mean Square Error}
\newacronym{roi}{ROI}{Region of Interest}
\newacronym{ros}{ROS}{Robot Operating System}
\newacronym{rov}{ROV}{Remotely Operated Vehicle}
\newacronym{rpm}{RPM}{Revolutions Per Minute}
\newacronym{rrm}{RRM}{Regularized Risk Minimization}
\newacronym{rrt}{RRT}{Rapidly Exploring Random Tree}
\newacronym{rsme}{RSME}{Root-Square Mean Error}
\newacronym{rss}{RSS}{Relative State Specification}
\newacronym{rti}{RTI}{Real-Time Iteration}

%-----S-----%
\newacronym{sam}{SAM}{Small and Affordable Maritime Robot}
\newacronym{sbl}{SBL}{Short Baseline}
\newacronym{sbp}{SBP}{Sub-bottom Profiler}
\newacronym{sdg}{SDG}{Sustainable Development Goal}
\newacronym{se}{SE}{Squared Exponential}
\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
\newacronym{sig}{SIG}{Static Interaction Graph}
\newacronym{sindy}{SINDY}{Sparse Identification of Nonlinear Dynamics}
\newacronym{slam}{SLAM}{Simultaneous Localization and Mapping}
\newacronym{smarc}{SMaRC}{Swedish Maritime Robotics Center}
\newacronym{sod}{SoD}{Subset of Data}
\newacronym{sofar}{SOFAR}{Sound Fixing And Ranging}
\newacronym{sqp}{SQP}{Sequential Quadratic Program}
\newacronym{svm}{SVM}{Support Vector Machine}

%-----T-----%
\newacronym{tcg}{TCG}{Transversal Center of Gravity}
\newacronym{tcp}{TCP}{Tool Center Point}
\newacronym{td}{TD}{Temporal Difference}
\newacronym{tms}{TMS}{Tether Management System}
\newacronym{tvg}{TVG}{Time Varied Gain}


%-----U-----%
\newacronym{uav}{UAV}{Unmanned Aerial Vehicle}
\newacronym{ude}{UDE}{Universal Differential Equation}
\newacronym{usbl}{USBL}{Ultra-Short Baseline}
\newacronym{usc}{USC}{Underwater Sound Channel}
\newacronym{usv}{USV}{Unmanned Surface Vehicle}
%-----V-----%
\newacronym{vbs}{VBS}{Variable Buoyancy System}
\newacronym{vc}{VC}{Vapnik-Chervonenkis}
\newacronym{vta}{VTA}{Visual Tracking Algorithm}
%-----W-----%
%-----X-----%
%-----Y-----%
%-----Z-----%
\newacronym{zoro}{zoRO}{Zero Order Robust Optimization}
